A systematic search for outbursting AM CVn systems with the Zwicky Transient Facility

AM CVn systems are a rare type of accreting binary that consists of a white dwarf and a helium-rich, degenerate donor star. Using the Zwicky Transient Facility (ZTF), we searched for new AM CVn systems by focusing on blue, outbursting stars. We first selected outbursting stars using the ZTF alerts. We cross-matched the candidates with $Gaia$ and Pan-STARRS catalogs. The initial selection of candidates based on the $Gaia$ $BP$-$RP$ contains 1751 unknown objects. We used the Pan-STARRS $g$-$r$ and $r$-$i$ color in combination with the $Gaia$ color to identify 59 high-priority candidates. We obtained identification spectra of 35 sources, of which 18 are high priority candidates, and discovered 9 new AM CVn systems and one magnetic CV which shows only He-II lines. Using the outburst recurrence time, we estimate the orbital periods which are in the range of 29 to 50 minutes. We conclude that targeted followup of blue, outbursting sources is an efficient method to find new AM CVn systems, and we plan to followup all candidates we identified to systematically study the population of outbursting AM CVn systems.

==> leftovertext.tex <==
The goal of this work is to determine if and how AM CVn systems can be identified using variability information and colour information. Here, we discuss the efficiency and completeness of this method.

As can be seen in Fig. \ref{fig:colorplots} and \ref{fig:venn}, AM CVn systems are typically more blue compared to the overall population of outbursting stars. Of the known AM CVn systems, 61 out of 67 (91\%) pass our first criterion ($BPRP<0.6$), but also passes 214 objects which are not AM CVn systems and 1736 unidentified objects. While this initial selection is relatively complete, there are too many unidentified objects to followup using longslit spectroscopy.

The strict selection criteria are an attempt to further reduce the number of candidates. As can be seen in Fig. \ref{fig:colorplots}, AM CVn systems also tend to be blue in the $g-r$ and $r-i$ colors. However, only half of the AM CVn systems pass these additional criteria. It does reduce the number of candidates by an order of magnitude. 


We compare the long-timescale behaviour of the 8 new systems with the sample in \citet{levitan2015} who used PTF to find outbursting AM CVn systems. If we compare the outburst recurrence times, we notice that the recurrence time of AM CVn systems in this work are noticeably longer. To illustrate this point, the shortest recurrence time of the systems in this work 130 days. In the PTF sample, 7 out of 11 systems show recurrence times \textit{shorter} than this.
This is likely due to two reasons. The first is that frequently outbursting systems are easier to discover and therefore most of them are already known. The second as been mentioned above


% gaia distances
\subsection{Evaluation of the selection criteria}
The goal of this work is to determine if and how AM CVn systems can be identified using variability information and colour information. Here, we briefly discuss the completeness, efficiency, and biases of this method. 


To select outbursting stars we used only ZTF, which has only been in operation for three years. While the ZTF cadence should be high enough to catch any outbursting star in its footprint, systems which have long outburst recurrence times are unlikely to be observed with ZTF. Other surveys like CRTS, PTF, and ATLAS have been observing the sky much longer. Adding the outburstings stars discovered by these surveys can significantly improve the completeness of the search, especially for long period systems.

% 1.5 magnitude outbursts?
The initial colour selection ($BP-RP<0.6$) is very broad and contains all known AM CVn systems. However, the selection criteria used to prioritise targets is very strict. While this eliminates many false positives, there are six outbursting AM CVn systems, including one of the newly discovered ones, which do not pass these selection criteria. 

This has two reasons. The first is that in long-period systems, the white dwarf is relatively cold and a small amount of emission from the disc can make the system appear to red. 
The second is due to the combination of outbursts and non-simultaneous observations. If the objects is observed in outburst in one band and in quiescence in the other, this can drastically alter the colour. The solution for this is to use the ZTF data use only the data obtained in quiescence to measure the color.


